OlaGPT: Empowering LLMs With Human-like Problem-Solving Abilities

In most current research, large language models (LLMs) are able to perform reasoning tasks by generating chains of thought through the guidance of specific prompts. However, there still exists a significant discrepancy between their capability in solving complex reasoning problems and that of humans. At present, most approaches focus on chains of thought (COT) and tool use, without considering the adoption and application of human cognitive frameworks. It is well-known that when confronting complex reasoning challenges, humans typically employ various cognitive abilities, and necessitate interaction with all aspects of tools, knowledge, and the external environment information to accomplish intricate tasks. This paper introduces a novel intelligent framework, referred to as OlaGPT. OlaGPT carefully studied a cognitive architecture framework, and propose to simulate certain aspects of human cognition. The framework involves approximating different cognitive modules, including attention, memory, reasoning, learning, and corresponding scheduling and decision-making mechanisms. Inspired by the active learning mechanism of human beings, it proposes a learning unit to record previous mistakes and expert opinions, and dynamically refer to them to strengthen their ability to solve similar problems. The paper also outlines common effective reasoning frameworks for human problem-solving and designs Chain-of-Thought (COT) templates accordingly. A comprehensive decision-making mechanism is also proposed to maximize model accuracy. The efficacy of OlaGPT has been stringently evaluated on multiple reasoning datasets, and the experimental outcomes reveal that OlaGPT surpasses state-of-the-art benchmarks, demonstrating its superior performance. Our implementation of OlaGPT is available on GitHub: \url{https://github.com/oladata-team/OlaGPT}.

==> relatedwork.tex <==
\section{RELATED WORK}
\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.4]{images/architecture.png}
    \caption{Three stages of black/grey industries}
    \label{architecture}
\end{figure*}
\subsection{Augmented Language Model}
Augmented language model usually refers to the enhancement of a large language model's reasoning skills and the ability to use tools. The former is defined as decomposing a potentially complex task into simpler subtasks while the latter consists in calling external modules. 
% Prompt engineering refers to the method of using prompt techniques to guide its generation behavior without updating the weight of the model, so as to achieve the goal as much as possible. Relying on a large amount of human experience, the same prompt has large differences in different models.
% prompt engineering
Among prompt engineering methods, Chain-of-Thought (CoT) prompting \cite{wei2023chainofthought} is a popular technique that does not require fine-tuning model parameters. It is particularly effective in improving the model's performance in complex reasoning questions by simply changing the input. \cite{diao2023active} references uncertainty-based active learning to mine most uncertain questions, which are then manually annotated and iteratively selected to stimulate reasoning ability as much as possible. To reduce the cost of manual annotation, a fully automated pipeline named  Automate-CoT (Automatic Prompt Augmentation and Selection with Chain-of-Thought) is proposed in \cite{shum2023automatic}, which uses a variance-reduced policy gradient strategy to estimate the significance of each example in LLM. Another automatic CoT prompting method: Auto-CoT \cite{zhang2022automatic} samples questions with diversity and generates reasoning chains to construct prompt. Additionally, a solution is proposed in \cite{wang2023selfconsistency} to improve the results by using a voting strategy to select the most consistent answer output based on the results generated from different reasoning paths. Automatic Reasoning and Tool-use (ART) \cite{paranjape2023art} uses frozen LLMs to automatically generate intermediate reasoning steps as a program. This framework selects demonstrations of multi-step reasoning and tool use from a task library.Self-Taught Reasoner (STaR)\cite{zelikman2022star} relies on a simple loop: if the generated answers are wrong, try again to generate a rationale given the correct answer; fine-tune on all the rationales that ultimately yielded correct answers.
Few-shot prompting struggles as task complexity increases. Consequently, many recent works employ in-context learning to decompose complex problems into sub-problems and effectively teach these sub-problems via separate prompts, such as SeqZero\cite{yang2022seqzero},Decomposed Prompting\cite{khot2023decomposed}.
% tool use
Although recent LLMs are able to correctly decompose many problems, they are still prone to errors when dealing with performing complex arithmetics. Program-Aided Language models (PAL) \cite{gao2023pal} decompose symbolic reasoning, mathematical reasoning, or algorithmic tasks into intermediate steps along with python code for each step.Similarly, \cite{Drori_2022} prompts Codex\cite{chen2021evaluating} to generate executable code-based solutions to university-level problems. furthermore, \cite{schick2023toolformer} introduces Toolformer, a model trained to decide which APIs to call, when to call them, what arguments to pass, and how to best incorporate the results into future token prediction.

\subsection{Cognitive Architecture}
\cite{kotseruba202040} discusses the development of cognitive architectures over the past four decades, focusing on their core cognitive abilities and the practical applications that have emerged from this research. This summary highlights the core cognitive abilities of these architectures and their practical applications in various domains.
Perception: Cognitive architectures have been designed to model human perception, including visual, auditory, and tactile modalities. These models have been used to study how humans process and interpret sensory information, leading to insights into attention, pattern recognition, and object recognition.

Memory: Memory is a critical component of cognitive architectures, as it allows the system to store and retrieve information. Researchers have developed models of short-term and long-term memory, as well as episodic and semantic memory, to better understand how humans encode, store, and retrieve information.

Learning: Learning is a fundamental aspect of human cognition, and cognitive architectures have been developed to model various learning processes, such as reinforcement learning, supervised learning, and unsupervised learning. These models have provided insights into how humans acquire new knowledge and skills, as well as how they adapt to changing environments.

Problem-solving: Cognitive architectures have been used to model human problem-solving abilities, including planning, reasoning, and decision-making. These models have been applied to a wide range of tasks, from simple puzzles to complex real-world problems, providing insights into the cognitive processes underlying human problem-solving.

Decision-making: Decision-making is a critical aspect of human cognition, and cognitive architectures have been developed to model various decision-making processes, such as risk assessment, choice, and judgment. These models have been used to study how humans make decisions in various contexts, including economic, social, and environmental situations.
